The Effectiveness of Edge Detection Evaluation Metrics for Automated Coastline Detection

We analyse the effectiveness of RMSE, PSNR, SSIM and FOM for evaluating edge detection algorithms used for automated coastline detection. Typically, the accuracy of detected coastlines is assessed visually. This can be impractical on a large scale leading to the need for objective evaluation metrics. Hence, we conduct an experiment to find reliable metrics. We apply Canny edge detection to 95 coastline satellite images across 49 testing locations. We vary the Hysteresis thresholds and compare metric values to a visual analysis of detected edges. We found that FOM was the most reliable metric for selecting the best threshold. It could select a better threshold 92.6% of the time and the best threshold 66.3% of the time. This is compared RMSE, PSNR and SSIM which could select the best threshold 6.3%, 6.3% and 11.6% of the time respectively. We provide a reason for these results by reformulating RMSE, PSNR and SSIM in terms of confusion matrix measures. This suggests these metrics not only fail for this experiment but are not useful for evaluating edge detection in general.

==> archive.tex <==

\begin{figure}[h]
\centering
\includegraphics[width=0.99\textwidth]{figures/rmse.png}
\caption{Average RMSE for each spectral band with error bars given by the standard deviation. For each band, the performance improves as we increase the thresholds. Overall, the NIR band is the worst-performing band.}
\label{fig:rmse}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.99\textwidth]{figures/psnr.png}
\caption{Average PSNR for each spectral band with error bars given by the standard deviation. For each band, the performance improves as we increase the thresholds. Overall, the NIR band is the worst-performing band. }
\label{fig:psnr}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.99\textwidth]{figures/ssim.png}
\caption{Average SSIM for each spectral band with error bars given by the standard deviation. For each band, the performance improves as we increase the thresholds. }
\label{fig:ssim}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.99\textwidth]{figures/fom.png}
\caption{Average FOM for each spectral band with error bars given by the standard deviation. For each band, there is an initial improvement followed by a decrease in average performance.}
\label{fig:fom}
\end{figure}

Table~\ref{tab:nir_results} gives the average metric values at each threshold for the NIR band. When using  the highest thresholds tend to produce the best results. 
\input{figures/nir_table.tex}




==> figures/nir_table.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Threshold 1} & \textbf{Threshold 2} & \textbf{RMSE}  & \textbf{PSNR}  & \textbf{SSIM} & \textbf{FOM}  \\ \hline
50                   & 100                  & 74.02          & 11.06          & 0.7           & 0.31          \\ \hline
50                   & 150                  & 67.16          & 11.92          & 0.75          & 0.34          \\ \hline
100                  & 200                  & 55.93          & 13.48          & 0.82          & 0.4           \\ \hline
100                  & 300                  & 48.23          & 14.76          & 0.86          & \textbf{0.42} \\ \hline
200                  & 400                  & 39.83          & 16.39          & 0.9           & 0.33          \\ \hline
200                  & 600                  & \textbf{35.94} & \textbf{17.27} & \textbf{0.91} & 0.14          \\ \hline
\end{tabular}
\end{center}
\caption{Average metrics across the 98 test images for the NIR spectral band. For each metric, the best average is given in bold. For RMSE, RSNR and SSIM, the performance of canny edge detection tends to improve as we increase the thresholds.  For FOM there is an initial improvement and then a decrease in performance. }
\label{tab:nir_results}
\end{table}
